Predicting Livelihood Indicators from Community-Generated Street-Level Imagery

Major decisions from governments and other large organizations rely on measurements of the populace's well-being, but making such measurements at a broad scale is expensive and thus infrequent in much of the developing world. We propose an inexpensive, scalable, and interpretable approach to predict key livelihood indicators from public crowd-sourced street-level imagery. Such imagery can be cheaply collected and more frequently updated compared to traditional surveying methods, while containing plausibly relevant information for a range of livelihood indicators. We propose two approaches to learn from the street-level imagery: (1) a method that creates multi-household cluster representations by detecting informative objects and (2) a graph-based approach that captures the relationships between images. By visualizing what features are important to a model and how they are used, we can help end-user organizations understand the models and offer an alternate approach for index estimation that uses cheaply obtained roadway features. By comparing our results against ground data collected in nationally-representative household surveys, we demonstrate the performance of our approach in accurately predicting indicators of poverty, population, and health and its scalability by testing in two different countries, India and Kenya. Our code is available at https://github.com/sustainlab-group/mapillarygcn.

==> sections/impact.tex <==
\section*{Statement of Broader Impact}
International aid organizations and governments must be able to measure a populace's well-being to understand where assistance is needed, but traditional ground-based survey methods used to collect data on well-being are expensive and time-consuming. Thus, several years or even decades will pass between surveys in some countries, inhibiting the ability of many organizations to understand or improve well-being. Although recent innovations in machine learning offer promising approaches to faster and more inexpensive livelihood measurement, the adoption of these new approaches by organization on the ground has been inhibited by their lack of interpretability: model-based features are typically not semantically meaningful, and practitioners on the ground are understandably hesitant to substitute these predictors for ones they understand. 

This work presents the first use of new crowdsourced street-level imagery from Mapillary for the task of predicting key livelihood indicators at a local level. 
We show how this relatively cheap and growing data source generated by citizens can be used to train models that learn to predict a variety of indicators in spite of the imagery's inconsistent and noisy quality. We then demonstrate how to visualize the models to understand what features are important in predictions. %Currently, the DHS performs wealth index estimation by documenting what assets an individual household owns, what material was used for construction, where it sources water and light, etc. and performing PCA. 
We show how objects detectable from the road can provide fine-grained, accurate estimates as well for a much cheaper cost and how certain objects signal development, growth, or economic activity.

While our livelihood labels derive from high-quality nationally representative data and are unlikely to be biased, there are possible biases in our crowd-sourced imagery because users upload images captured while driving, so coverage may be better alongside developed roads. Additionally, users do need a camera or a phone with camera to take the photos. However, since anyone can upload images and Mapillary supports past versions of Android and iOS, there is a diverse range of imagery uploaded from rural and developed areas across the country. Furthermore, we ensure user privacy as Mapillary blurs out faces, and our ground data contain anonymized information on dozens of households per village and thus are not individually traceable. 
%In the case a user hacked the model and, for example, disproportionately added images in various areas to change estimates, we could

Our research establishes new benchmarks for performance on the task of predicting livelihood indicators from crowd-sourced street-level imagery. We demonstrate our approach's ability to make predictions on poverty, population density, and even a health-related measure that may not be obvious or intuitive from imagery, i.e. women's body-mass index (a key nutritional indicator). We also show our method scales to all of India, one of the most populous and economically diverse countries in the world. As Mapillary offers coverage throughout the developing world, we believe our pipeline can be generalized both geographically and to other livelihood-specific tasks, amplifying the efficacy of a range of humanitarian and sustainability organizations in need of this type of data. % and help the end-user organizations measure progress more frequently and extend their reach to areas currently linked by poor infrastructure.
